Learning Joint Semantic Parsers from Disjoint Data

We present a new approach to learning semantic parsers from multiple datasets, even when the target semantic formalisms are drastically different, and the underlying corpora do not overlap. We handle such "disjoint" data by treating annotations for unobserved formalisms as latent structured variables. Building on state-of-the-art baselines, we show improvements both in frame-semantic parsing and semantic dependency parsing by modeling them jointly.

==> text/7-related_work.tex <==
\section{Related Work}
\label{sec:related}

%\sam{I moved this section earlier, and I think we should talk about \citet{peng2017deep} here.}

\paragraph{Semantic role labeling.}
% Much effort has been devoted to frame semantic parsing since \citet{gildea2002srl}, 
% including both feature-rich models \interalia{johansson2007lth,das2010probabilistic,das2012exact,das2014frame}
% and more recent ones that use representation learning \citep{swayamdipta2017frame}.
There is a parallel line of work on PropBank-style semantic role labeling, 
and several notable ones among them include \interalia{koomen2005generalized,roth2016neural,collobert2011nlp,zhou2015end2end,he2017deep}.
Due to the similarities between FrameNet and PropBank, 
algorithms devised for one of them can often be adapted to the other \interalia{tackstrom2015efficient,fitzgerald2015semantic,yang2017joint}.

%\citet{roth2014composition}\\
%\citet{belanger2017end2end}\\
%\citet{toutanova2008global}\\


\paragraph{Joint learning for NLP.}
Recent advances in representation learning drastically extend
earlier explorations of parameter sharing \citep{ando2005framework,blitzer-06,daume2007frustratingly}
in joint learning of multiple NLP tasks \citep{collober2008unified,zhang2016stack,soggard2016deep},
among different languages \citep{ammar2016many,guo2016universal},
and across domains \citep{johansson2013training,kshirsagar2015frame,kim2016frustratingly}.
Another line of work uses factors
across multiple tasks \citep{sutton2005joint,naradowsky2012improving,lluis2013joint,lewis2015joint}.
